Parameter Adaptation and Criticality in Particle Swarm Optimization

Generality is one of the main advantages of heuristic algorithms, as such, multiple parameters are exposed to the user with the objective of allowing them to shape the algorithms to their specific needs. Parameter selection, therefore, becomes an intrinsic problem of every heuristic algorithm. Selecting good parameter values relies not only on knowledge related to the problem at hand, but to the algorithms themselves. This research explores the usage of self-organized criticality to reduce user interaction in the process of selecting suitable parameters for particle swarm optimization (PSO) heuristics. A particle swarm variant (named Adaptive PSO) with self-organized criticality is developed and benchmarked against the standard PSO. Criticality is observed in the dynamic behaviour of this swarm and excellent results are observed in the long run. In contrast with the standard PSO, the Adaptive PSO does not stagnate at any point in time, balancing the concepts of exploration and exploitation better. A software platform for experimenting with particle swarms, called PSO Laboratory, is also developed. This software is used to test the standard PSO as well as all other PSO variants developed in the process of creating the Adaptive PSO. As the software is intended to be of aid to future and related research, special attention has been put in the development of a friendly graphical user interface. Particle swarms are executed in real time, allowing users to experiment by changing parameters on-the-fly.

==> sections/formulation.tex <==
\chapter{Formulation of the Problem \& Proposed Solution}

\section{Current Solutions}

In order to make databases easier to use for everyone we must first work out
why they are difficult to use and how current solutions fall short in the first
place. We see that most current database front-ends are either custom built or
ugly general purpose table-styled editors that make any meaningful edits hard
to comprehend.

\subsection{Bespoke Software}

The custom built solutions usually don't look anything like a database
and often, on the contrary, completely hide the fact that there is
a database powering them. Web applications such as \emph{Facebook} are
classic examples of this: behind the scenes there will be databases
holding and retrieving information but there will never be a single
mention of a select, join, table, or view on the front end for the user
to contend with.

There are clear advantages to showing the database in this manner.
Assuming that the front end is well designed and accessible, any user
will be able to perform all of the required actions on the stored data.
This also includes operations that are would be fantastically complex if
they needed to be typed out as a collection of huge \ac{SQL} statements
surrounded by a transaction. Instead, they are just a button on a web
page.

The problem with applying this solution to the database accessibility
problem is how specific and bespoke it is. We are unable to generalise
this beyond very simple cases due to the varying scales and types of
data stored. In addition, these solutions are expensive and time
consuming to create each time a new schema is used and data to display
and manipulate.

\subsection{General Purpose Software}

A compromise needs to be found between these two extremes: user-friendly
but bespoke and hard-to-use but powerful. In order to find this
compromise I am going to present the user with a new type of view of the
database that they are already familiar with: a file and directory tree.

This representation makes sense from a familiarity perspective as nearly
all computer users will have at some point had experience of using
a file tree. It additionally makes sense when applied to the structure
of a database too. \acf{DBMS} have a shallow tree structure when
representing the hierarchy of a server, database, table, and records.
A file tree is a simple way of displaying this structure that the user
is familiar with.

A further advantage of using the files and directories representation is
that it also allows the user to not just manipulate the files and
directories but also modify their contents. This allows us to present
the data to the user in a program that they are familiar with such as an
office package.

\section{Proposed Solution}

A good compromise needs to be found between these two extremes:
user-friendly but bespoke and hard-to-use but powerful. In order to find
this compromise I am going to present the user with a new type of view
of the database that they are already familiar with: a file and
directory tree.

This representation makes sense from a familiarity perspective as nearly
all computer users will have at some point had experience of using
a file tree. It additionally makes sense when applied to the structure
of a database too. \acf{DBMS} have a shallow tree structure when
representing the hierarchy of a server, database, table, and records.
A file tree is a simple way of displaying this structure that the user
is familiar with.

A further advantage of using the files and directories representation is
that it also allows the user to not just manipulate the files and
directories but also modify their contents. This allows us to present
the data to the user in a program that they are familiar with such as an
office package.

